LDPC Code Design for Transmission of Correlated Sources Across Noisy Channels Without CSIT

We consider the problem of transmitting correlated data after independent encoding to a central receiver through orthogonal channels. We assume that the channel state information is not known at the transmitter. The receiver has access to both the source correlation and the channel state information. We provide a generic framework for analyzing the performance of joint iterative decoding, using density evolution. Using differential evolution, we design punctured systematic LDPC codes to maximize the region of achievable channel conditions, with joint iterative decoding. The main contribution of this paper is to demonstrate that properly designed LDPC can perform well simultaneously over a wide range of channel parameters.

==> bsc_correlation.tex <==
Consider a symmetric correlation model which can be defined in terms of
a single parameter. For binary sources $U_1$ and $U_2$, this parameter
is given by $\Pr(U_1=U_2)$. It is useful to visualize this
correlation by the presence of an auxiliary binary symmetric channel
(BSC) with parameter $1-p$ between the sources. In other words, $U_2$ is
the output of a BSC with input $U_1$ i.e., $U_2 = U_1 + Z$. Here
$Z$ is a Bernoulli-($1-p$) random variable and can be thought of as an
{\em error}. Let $h_2(\cdot)$ denote the binary entropy function. Then,
$\entropy{U_1|U_2} = \entropy{U_2|U_1} = h_2(p)$ and $\entropy{U_1,U_2}
= 1 + h_2(p)$.

This correlation model can be incorporated into the Tanner graph at the
decoder (described in Section~\ref{sec:ldpc-codes}) as check nodes
between the source bits, with a hidden node representing the auxiliary
random variable $Z$ (which carries a constant log-likelihood ratio
$\log\frac{1-p}{p}$) attached to the check node. For this scenario, the
decoder does not require any side information i.e., it does not need to
know the realization of the auxiliary random variable $Z$.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "istc10"
%%% End: 

